Base Change for the Iwahori-Hecke Algebra of GL_2

Let $F$ be a non-Archimedean local field of characteristic not equal to 2, let $E/F$ be a finite unramified extension field, and let $\sigma$ be a generator of $\text{Gal}(E, F )$. Let $f$ be an element of $Z(H_{I_E})$, the center of the Iwahori-Hecke algebra for $GL_2(E)$, and let $b$ be the Iwahori base change homomorphism from $Z(H_{I_E})$ to $Z(H_{I_F})$, the center of the Iwahori-Hecke algebra for $GL_2(F)$ [8]. This paper proves the matching of the $\sigma$-twisted orbital integral over $GL_2(E)$ of $f$ with the orbital integral over $GL_2(F)$ of $bf$. To do so, we compute the orbital and $\sigma$-twisted orbital integrals of the Bernstein functions $z_{\mu}$. These integrals are computed by relating them to counting problems on the set of edges in the building for $SL_2$. Surprisingly, the integrals are found to be somewhat independent of the conjugacy class over which one is integrating. The matching of the integrals follows from direct comparison of the results of these computations. The fundamental lemma proved here is an important ingredient in the study of Shimura varieties with Iwahori level structure at a prime $p$ [7].

==> Copyright.tex <==
%Copyright

\thispagestyle{empty}
\hbox{\ }

\vfill
\renewcommand{\baselinestretch}{1}
\small\normalsize

\vspace{-.65in}

\begin{center}
\large{\copyright \hbox{ }Copyright by\\
Walter Randolph Ray-Dulany  %Type your name as it appears in University records
\\
2010}
\end{center}

\vfill

